LLM as Prompter: Low-resource Inductive Reasoning on Arbitrary Knowledge Graphs

Knowledge Graph (KG) inductive reasoning, which aims to infer missing facts from new KGs that are not seen during training, has been widely adopted in various applications. One critical challenge of KG inductive reasoning is handling low-resource scenarios with scarcity in both textual and structural aspects. In this paper, we attempt to address this challenge with Large Language Models (LLMs). Particularly, we utilize the state-of-the-art LLMs to generate a graph-structural prompt to enhance the pre-trained Graph Neural Networks (GNNs), which brings us new methodological insights into the KG inductive reasoning methods, as well as high generalizability in practice. On the methodological side, we introduce a novel pretraining and prompting framework ProLINK, designed for low-resource inductive reasoning across arbitrary KGs without requiring additional training. On the practical side, we experimentally evaluate our approach on 36 low-resource KG datasets and find that ProLINK outperforms previous methods in three-shot, one-shot, and zero-shot reasoning tasks, exhibiting average performance improvements by 20%, 45%, and 147%, respectively. Furthermore, ProLINK demonstrates strong robustness for various LLM promptings as well as full-shot scenarios.

==> sections/relatedwork.tex <==
\section{Detailed Related Work}
\label{sec:relatedwork}

\subsection{KG Inductive Reasoning}
Traditional \emph{transductive} KG embedding models, represented by TransE \cite{TransE}, DistMult \cite{DistMult-paper} and RotatE \cite{RotatE}, learn continuous vectors in the embedding space to represent each entity and relation in the knowledge graph. 
%However, these models operate on the premise that all entities and relations in the knowledge graph are known beforehand, and lack generalization capabilities for new entities within the same graph or across different KGs~\cite{2017Survey,GoogleAttH,OurRotL}. 
In contrast, KG \emph{inductive} reasoning methods~\cite{NBF-NIPS21} overcome this limitation by generalizing to KGs with unseen entities or relations.
Most existing inductive methods \cite{Cycle-ICML22,InductivE-IJCNN21,IKR-JWWW23,TACT-AAAI21} leverage Graph Neural Networks (GNN) to generate ``relative'' entity embeddings, by extracting local structural features from an induced graph of the query entity.
GraIL \cite{GraIL-ICML19} extracts an enclosing subgraph between the query entity and each candidate entity, but suffers from high computational complexity. 
NBFNet \cite{NBF-NIPS21} and RED-GNN \cite{REDGNN-WWW22} propagate query features through the $L$-hop neighborhood subgraph of the query entity. 
% To further enhance model efficiency, recent studies have focused on algorithmic improvements, including path-pruning methods in the GNN propagation process \cite{AdaProp-Arxiv22,OurGraPE}. 
%Despite these advancements, a significant limitation remains: 
These inductive methods struggle to generalize to KGs with new relation types, as the entity embeddings are still a function of a predetermined relation vocabulary.

\subsection{Few-shot and Unseen Relation Reasoning} 

To generalize to unseen relations, early efforts have explored meta-learning for few-shot link prediction, which predicts KG facts of unseen relations using a limited number of support triples \cite{FewKGR-EMNLP19,FewKGR-AAAI20,FewKGR-NIPS22,FewKGR-SIGKDD23,FewKGR-ICLR23}. 
However, those methods cannot work on an entire unseen inference graph.
Recent approaches focus on constructing graphs of relations to generalize to unseen relations \cite{rmpi,mtdea}. 
%RMPI~\cite{rmpi} transforms the surrounding subgraph of a triple in the original KG into a new relation-view graph, then learns the embedding of an unseen relation from the relational subgraph. 
InGram~\cite{ingram} relies on a featurization strategy based on the discretization of node degrees, which is effective only for KGs with a similar relational distribution and falls short in transferring to arbitrary KGs.
ISDEA~\citep{isdea} utilizes relation exchangeability in multi-relational graphs, which imposes stringent assumptions on the class of transferable relations coming from the same distribution. 
ULTRA \cite{ultra} employs a pre-training and fine-tuning framework, with a global relation graph extracted from the entire set of KG triples. 
However, the effectiveness of the above methods is contingent on sufficient support triples for the unseen relations in the inference KG, struggling with few-shot relation types in low-resource scenarios that limit their applicability.

\subsection{Text-based methods via Language Models}
%In recent years, the AI community has witnessed the emergence of numerous powerful pre-trained language Models (PLMs), such as BERT~\citep{Bert}, Llama-2~\citep{Llama2}, and GPT-4~\citep{Gpt4} which are driving huge advancements and lead to the pursuit of possible Artificial General Intelligence (AGI) \cite{brown2020language,ouyang2022training,bubeck2023sparks}.
A line of text-based KG inductive reasoning methods like BLP~\citep{TextKGR-BLP-WWW21}, KEPLER~\citep{TextKGR-KEPLER-TACL21}, StATIK~\citep{TextKGR-StATIK-NAACL21}, RAILD~\citep{TextKGR-RAILD-IJCKG22} rely on textual descriptions of entities and relations and use pre-trained language models (PLMs) like BERT~\citep{Bert} to encode them. 
To seek higher prediction performance, current methods mostly prefer to fine-tune PLMs which requires high computational complexity and limits its generalizability to other KGs with different formats of textual descriptions.
CSProm-KG \cite{CSPromKG-ACL23} and PDKGC \cite{PDKGC-arxiv23} perform KG link prediction via a frozen PLM with only the prompts trained. 
By combining graph structure features and textual representations, these methods perform well in transductive KG reasoning tasks. However, the trainable prompts are tuned for a fixed relation vocabulary and cannot be generalized to inductive reasoning.
Recent work \cite{LLMKGC-23arxiv} verifies the reasoning performance of large language models by converting a query into textual names of the query entity and relation.
We consider this family of methods to be orthogonal to our work. 
Our approach operates under the low-resource assumption that the graphs lack explicit entity descriptions, focusing instead on leveraging structural graph information and relation descriptions. 

% Our approach is significantly enhanced by the capabilities of powerful large language models. These models facilitate the understanding of relation descriptions across diverse domains, thereby supporting low-resource reasoning on domain-specific graphs.

% By reusing memorized knowledge from pre-training, PLM-based KGC methods can estimate unseen links without infering them from seen links in the target KG. A recent study \cite{PLMKGC-arxiv23} constructed synthetic datasets to analyze the performance of KG reasoning in pre-trained language model (PLM)-based methods. It has concluded that PLMs not only reuse memorized knowledge but also acquire essential inference abilities tailored for effective KG reasoning.


